What Makes a Good Team? A Large-scale Study on the Effect of Team Composition in Honor of Kings

Team composition is a central factor in determining the effectiveness of a team. In this paper, we present a large-scale study on the effect of team composition on multiple measures of team effectiveness. We use a dataset from the largest multiplayer online battle arena (MOBA) game, Honor of Kings, with 96 million matches involving 100 million players. We measure team effectiveness based on team performance (whether a team is going to win), team tenacity (whether a team is going to surrender), and team rapport (whether a team uses abusive language). Our results confirm the importance of team diversity and show that diversity has varying effects on team effectiveness: although diverse teams perform well and show tenacity in adversity, they are more likely to abuse when losing than less diverse teams. Our study also contributes to the situation vs. personality debate and show that abusive players tend to choose the leading role and players do not become more abusive when taking such roles. We further demonstrate the predictive power of features based on team composition in prediction experiments.

==> main.tex <==


\section{the influence of roles-combination on other aspects}
The influence of roles combination can also be reflected from abusing and surrendering behavior. Here we would simply introduce the abusing and surrendering phenomenon in the game, where players can choose to talk or type with teammates, and they can launch the surrendering; if 4 of 5 players agree, the camp would lose at once, no matter the current game condition.

\begin{figure}[h!]
	\centering
	\subfigure[abuse-scale distribution]{
		\includegraphics[width=0.2\textwidth]{abuse_scale_distribution.pdf}
		\label{fig:abuse scale dist}
	}
	\subfigure[abuse-proportion vs abuse-scale]{
		\includegraphics[width=0.2\textwidth]{abuse_corr_scale.pdf}
		\label{fig:abuse corr scale}
	}
	%\hspace{0.5in}
	%\hspace{0.5in}
	\caption{abusing-scale vs roles-combination}
	\label{fig:abuse corr-scale}
\end{figure}


\subsection{Surrendering Combinations}


\section{the variety of roles in the combinations}
In this section, we would answer the question that which roles combinations are more abusive, or more likely to surrender. From our observations, the variety of roles in the combinations greatly influence the team performance.



\section{Individual Influence of Roles on the team}
In sections above, we've focused on the overall impact of roles combinations on the team performance, and in this section, we'll explore the individual influence of roles on abusing and surrendering behavior.

\subsection{Surrendering Behavior}



